Generalized cross-resonance scheme for maximally-entangling two-qutrit gates

To utilize higher-dimensional quantum systems, in this Letter, we derive a generalized cross-resonance (GCR) scheme for realizing maximally entangling two-qutrit gates on fixed-frequency transmons beyond the 0-1 subspace. Our two-qutrit gates, namely, $U_{CR}^{01}$ and $U_{CR}^{12}$, acting on the $0{\text -}1$ and $1{\text -}2$ energy transitions of transmons, respectively, directly allow for entanglement on the $1{\text -}2$ levels. Unlike the known works, our gate is parametric in nature, enabling us to construct multiple entangling gates of interest. By performing simulations in Qiskit, we demonstrate two-qutrit generalized controlled-$X$ ($U_{CX}^{01}$ and $U_{CX}^{12}$) and controlled-$H$ ($U_{CH}^{01}$ and $U_{CH}^{12}$) gates, which are instances of the proposed $U_{CR}$ gates, with reported gate fidelities of $86.14\%~(99.73\%),~84.6\%~(97.88\%),~92.35\%~(99.39\%)$, and $91.99\%~(98.99\%)$, respectively with (and without) noise. We also reveal a two-qutrit Bell state with a fidelity of $99.06 \pm 0.01\%$, with a complete Bell state preparation in a $\sim514$ ns pulse sequence, which is less than the gate time of the known scheme by cross-Kerr-based entangling gates.

==> abstract-old.tex <==
Superconducting transmons, often truncated to two levels for qubit operations, have an inherent multi-level energy structure that offers untapped potential for higher-dimensional quantum systems like qutrits.
Three-level systems have natural advantages over their two-level counterparts in quantum information and computation.
However, universal qutrit computation requires high-fidelity entangling gates spanning all three levels, which remain experimentally challenging. 
In this letter, we introduce the generalized cross-resonance scheme (GCR) which is a comprehensive theoretical framework that generalize the qubit-centric cross-resonance (CR) interaction beyond the 0-1 subspace for realizing maximally entangling two-qutrit gates on fixed-frequency transmons and is a microwave-only technique compatible with existing hardware. 
We use the GCR scheme to design parametric two-qutrit gates, namely, $\ucrzeroone$ and $\ucronetwo$, that act on the $0{-}1$ and $1{-}2$ energy transitions of transmons. 
Our gates improve upon the existing works in two aspects.
First, our gates \emph{directly} allow for entanglement on the $1{-}2$ levels rather than merely relying on $0{-}1$ entanglement, as in previous works. Second, our gates are parametric in nature, enabling us to construct multiple entangling gates of interest, whereas the purview of prior works that use cross-resonance for qutrits was limited to individual gates. 
Using numerical simulation in Qiskit Dynamics, we demonstrate two-qutrit generalized controlled-$X$ ($\gcxzero$ and $\gcxone$) and controlled-$H$ ($\gcsqrtzero$ and $\gcsqrtone$) gates, which are instances of the proposed $\ucr$ gates, with reported gate fidelities of $99.73\pm 0.01\%, 97.88\pm 0.01\%, 99.39\pm 0.01\%$, and $98.99\pm 0.01\%$, respectively.
Finally, we prepare a two-qutrit Bell state $|\psi\rangle = \frac{1}{\sqrt{3}}(|00\rangle + |11\rangle + |22\rangle)$ with a fidelity of $99.06 \pm 0.01\%$. 
We note that, in our setup, the complete time taken for Bell state preparation is $\sim 514$ ns and is less than the gate time of cross-Kerr-based entangling gates. 

==> abstract.tex <==
Superconducting transmons, often truncated to two levels for qubit operations, have an inherent multi-level energy structure that offers untapped potential for higher-dimensional quantum systems like qutrits. Three-level systems have natural advantages over their two-level counterparts in quantum information and computation. However, universal qutrit computation requires high-fidelity entangling gates spanning all three levels, which remain experimentally challenging\cite{Goss2022-nature}. In our work, we present a comprehensive theoretical framework for realizing maximally entangling two-qutrit gates on fixed-frequency transmons that generalize the qubit-centric cross-resonance (CR) interaction beyond the 0-1 subspace, leading to a generalized cross-resonance (GCR) scheme, a microwave-only technique compatible with existing hardware. We use the GCR scheme to design parametric two-qutrit gates, namely, $\ucrzeroone$ and $\ucronetwo$, that act on the \(0-1\) and \(1-2\) energy transitions of transmons, respectively. These parametric gates induce state-dependent Rabi oscillations on the target qutrit’s \(0-1\) and \(1-2\) transitions, controlled by the state of the control qutrit. These gates are activated via amplitude-modulated Gaussian pulses with flat tops, leveraging microwave drives without requiring tunable couplers. Our gates improve upon the existing works in two aspects. First, our gates \emph{directly} allow for entanglement on the $1-2$ levels instead of relying on the entangling ability on the $0-1$ levels to perform entanglement on the subspace spanned by $|1\rangle $ and $|2\rangle $, as done in previous works \cite{Scrambling21,cervera2022experimental}. Second, our gates are parametric in nature, enabling us to construct multiple entangling gates of interest, while the prior works that use cross-resonance for qutrits \cite{Scrambling21,cervera2022experimental} focus on individual gates. Further, we use Qiskit Dynamics to perform a simulation-based demonstration of two-qutrit generalized controlled-$\sqrt{X}$ gates,  namely, $\gcsqrtzero$ and $\gcsqrtone$, which are instances of proposed $\ucr$ gates. Numerical simulations in Qiskit Dynamics, calibrated to experimental parameters that mimic the actual backend, demonstrate a maximal concurrence of \(97.2\pm0.1\% \), confirming entanglement across all three levels. A two-qutrit Bell state \(|\psi\rangle = \frac{1}{\sqrt{3}}(|00\rangle + |11\rangle + |22\rangle)\) is prepared with \(96.9 \pm 0.1\%\) fidelity using a 704 ns pulse sequence. We note that the complete time taken for Bell state preparation in our setup is at times less than the gate time of cross-Kerr-based entangling gates\cite{Goss2022-nature}.

